Implicit Deep Learning

Implicit deep learning prediction rules generalize the recursive rules of feedforward neural networks. Such rules are based on the solution of a fixed-point equation involving a single vector of hidden features, which is thus only implicitly defined. The implicit framework greatly simplifies the notation of deep learning, and opens up many new possibilities, in terms of novel architectures and algorithms, robustness analysis and design, interpretability, sparsity, and network architecture optimization.

==> authors.tex <==
% order to be determined later
L. El Ghaoui, B. Travacca, A. Tsai, F. Gu, A. Askari

==> feedback-connect.tex <==
\section{Feedback Connection of Implicit Models}
\label{app:feedback-connect}
In this section, we provide the details on the feedback connection of two implicit models, as mentioned at the end of~\cref{sub:composition}.

Assume that The model matrices are given by
\[
\left(\begin{array}{c|c} 
A & B \\\hline C & D
\end{array}\right) = 
\left(\begin{array}{cc|c} 
A_1 & B_1C_2 & B_1 \\ B_2C_1 & A_2 & 0 \\\hline
C_1 & 0 & 0
\end{array}\right).
\]

==> proof-gradients-exist.tex <==
\section{Proof of \cref{thm:grad_exist}} \label{app:grad_exist_proof}
From \cref{app:grad-descent}, we get the following closed form evaluation of gradients for ($A, B, C, D$).
$$
\nabla_M \cal L = \begin{pmatrix}
\nabla_A \cal L &
\nabla_B \cal L \\
\nabla_C \cal L &
\nabla_D \cal L \\
\end{pmatrix} = \begin{pmatrix}
\nabla_z \mathcal{L} \; x^\top &
\nabla_z \mathcal{L} \; u^\top \\
\nabla_{\hat{y}} \mathcal{L} \; x^\top &
\nabla_{\hat{y}} \mathcal{L} \; u^\top \\
\end{pmatrix},
$$
where $\nabla_{\hat{y}} \mathcal{L}$ can be easily computed and $\nabla_z\mathcal{L}$ can be given by the following equation.
$$
\nabla_z\mathcal{L} = \left(C (I - \tilde{D} A)^{-1} \tilde{D}\right)^\top \nabla_{\hat{y}} \mathcal{L}
$$
In the above equation, the matrix $(I - \tilde{D} A)^{-1}\tilde{D} = \frac{\partial x}{\partial z}$ is well-defined and unique. We show the existence and uniqueness by observing that the following equation (same as equation (\ref{eq:grad_key}) in derivation of $\frac{\partial x}{\partial z}$ given in \cref{app:grad-descent}) has a unique solution. Note that on the high level we are trying to put equation (\ref{eq:dummy_grad_implicit}) as an equilibrium equation (\ref{eq:eq-eq}) for some existing implicit model with well-posed $A$ and use the well-posedness to establish existence and uniqueness.
\begin{align}
    \frac{\partial x}{\partial z} &= \frac{\partial \phi(z)}{\partial z} + \frac{\partial \phi(Ax + Bu)}{\partial x} \cdot \frac{\partial x}{\partial z} = \tilde{D} + \tilde{D} A \cdot \frac{\partial x}{\partial z} \notag \\
    \frac{\partial x}{\partial z} &= \tilde{D} \left(A \cdot \frac{\partial x}{\partial z} + I\right) \notag \\
    \tilde{X} &= \tilde{D} \left(A \tilde{X} + I\right),\label{eq:dummy_grad_implicit}
\end{align}
where $\tilde{X} = \frac{\partial x}{\partial z}$. The above claim follows from 
\begin{enumerate}
    \item Matrix $A$ is well-posed for any CONE activation (resp. BLIP activation with fixed parameters $n_l$, $p_l$, $\gamma_l$, $l \in [L]$)
    \item (\cref{lem:d_wellposed}) If activation $\phi$ is CONE (resp. BLIP) then a new ``activation'',\\ $\tilde{\phi}(\cdot) = \tilde{D} (\cdot)$, defined by matrix multiplying $\tilde{D}$ with the input is also CONE (resp. BLIP with the same parameters $n_l$, $p_l$, $\gamma_l$, $l \in [L]$). 
    \item Slice $\tilde{X}$ and $I$ into columns and employ the well-posedness of $A$ on CONE (resp. BLIP) activation for each column. (\ie\;Unique solution $\tilde{x}_i$ exists for $\tilde{x}_i = \tilde{D}(A\tilde{x}_i + e_i), i\in[n]$, where $e_i$ is a $i$-th unit vector.)
\end{enumerate}
We conclude that each column of $\tilde{X}$ is existent and unique and that $\tilde{X} = (I - \tilde{D} A)^{-1}\tilde{D}$ is existent and unique.

\begin{lemma} \label{lem:d_wellposed}
If $\phi$ is CONE (resp. BLIP with fixed parameters $n_l$, $p_l$, $\gamma_l$, $l \in [L]$) then $\tilde{\phi}(\cdot) = \tilde{D} (\cdot)$ is also CONE (resp. BLIP with the same parameters $n_l$, $p_l$, $\gamma_l$, $l \in [L]$).
\end{lemma}
\begin{proof}
If $\phi$ is CONE, then $\tilde{D} = \frac{\partial \phi(z)}{\partial z}$ is diagonal or component-wise where $z \in \reals^n$ is the input to the activation $\phi$. And because $\phi$ is non expansive, $|\tilde{D}_{ii}| \le 1,  i \in [n]$. Thus
$$|\tilde{D}(u) - \tilde{D}(v)| = |\tilde{D} (u-v)| \le |\tilde{D}| |u-v| \le |u-v|, \;\;\forall u, v \in \reals^{n}, $$
meaning that the new ``activation'' $\tilde{\phi}(\cdot) = \tilde{D} (\cdot)$ which left multiplies any compatible input with $\tilde{D}$ is also non-expansive. We now conclude that $\tilde{\phi}(\cdot) = \tilde{D} (\cdot)$ is also CONE.

If $\phi$ is BLIP with fixed parameters $n_l$, $p_l$, $\gamma_l$, $l \in [L]$ (\ie\;For some input $z\in\reals^n$ partitioned as $z = (z_1, \dots, z_L), z_l\in \reals^{n_l}, l\in [L]$, $\phi(z) = (\phi_1(z_1), \dots, \phi_L(z_L))$.) , then $\tilde{D} = \frac{\partial \phi(z)}{\partial z} = \diag (\tilde{D}_1, \dots, \tilde{D}_L)$ is block diagonal with $\tilde{D}_l \in \reals^{n_l}$ and $\|\tilde{D}_l\|_{p_l} = \left\|\frac{\partial \phi_l(z_l)}{\partial z_l}\right\|_{p_l} \le \gamma_l$ for $l\in [L]$. The ``new'' activation $\tilde{\phi}(\cdot) = \tilde{D}(\cdot)$ can also be seen as blockwise by observing that $\tilde{\phi}(z) = (\tilde{\phi}_1(z_1), \dots,\tilde{\phi}_L(z_L)) = (\tilde{D}_1(z_1), \dots,\tilde{D}_L(z_L))  \tilde{D}(z)$. For the $l$-th block ``activation'' $\tilde{\phi}_l(\cdot) = \tilde{D}_l(\cdot)$, the following inequality holds.
$$\|\tilde{D}_l(u) - \tilde{D}_l(v)\|_{p_l} = \|\tilde{D}_l (u-v)\|_{p_l} \le \|\tilde{D}_l\|_{p_l}\|u-v\|_{p_l} \le \gamma_l \|u-v\|_{p_l}, \;\;\forall u, v \in \reals^{n_l}, $$
which shows that the new ``activation'' $\tilde{\phi}(\cdot)=\tilde{D}(\cdot)$ is blockwise and Lipschitz (BLIP) with the same parameters as that of $\phi$.
\end{proof}



==> proof-gradients-robust.tex <==
\section{Robust Gradient Descent}
\label{app:grad-descent-robust}
In this section, we consider robust implicit deep learning. In this case we are required to differentiate through a function of the form
\begin{align*}
f(A,B,C,D) = y^\top (|C|(I-|A|)^{-1}|B| + |D|)z
\end{align*}
where $|X|$ denotes taking entrywise absolute value of a matrix $X$. We are interested in calculating the gradient of $f$. First we note that 
\begin{align*}
g(|X|) = \nabla_X g(X) \circ \text{sgn}(X)
\end{align*}
where $X \circ Y$ denotes elementwise wise product of two matrices and $\text{sgn}(X)$ denotes taking the elementwise $\text{sgn}$ operation on each entry of the matrix (that is, $\text{sgn}(X)$ is a matrix whose entries are $\pm 1$ if the corresponding entry of $X$ is positive or negative, or $0$ if the entry of $X$ is 0). For completeness we would need to deal with subgradients here, but we choose to set the zero entries of $X$ to 0 in $\text{sgn}(X)$.

\paragraph{Calculating $\partial f/\partial A$} Let $g(X) = Tr(X^{-1} Q)$ where $Q = |B|zy^\top |C|$. Then $\partial f/\partial A = \partial g(I-A)/\partial A$. By the chain rule we have
\begin{align*}
\dfrac{\partial f}{\partial A_{ij}} = \sum_{k,l=1}^n \dfrac{\partial g(Z)}{\partial Z_{kl}} \dfrac{\partial Z_{kl}}{\partial A_{ij}}
\end{align*}
for $Z = I-A$. \\

Note $\partial Z_{kl}/\partial A_{ij} = -1$ if $(k,l) = (i,j)$ and $0$ otherwise. Furthermore, we have $\nabla_X g(X) = -(X^{-1} QX^{-1})^\top$. Hence
\begin{align*}
&\dfrac{\partial f}{\partial A_{ij}} = [\nabla_Z g(Z)]_{ij} \cdot (-1) \\
\Rightarrow &\dfrac{\partial f}{\partial A} = (Z^{-1} Q Z^{-1})^\top
\end{align*}

\paragraph{Calculating $\partial f/\partial B$} Let $q^\top  = y^\top |C|(I - |A|)^{-1}$. Then
\begin{align*}
\dfrac{\partial f}{\partial B} = qz^\top \circ \text{sgn}(B)
\end{align*}

\paragraph{Calculating $\partial f/\partial C$} Let $r = (I - |A|)^{-1} |B| z$. Then
\begin{align*}
\dfrac{\partial f}{\partial C} = yr^\top \circ \text{sgn}(C)
\end{align*}

\paragraph{Calculating $\partial f/\partial D$}
Trivially
\begin{align*}
\dfrac{\partial f}{\partial D} = yz^\top \circ \text{sgn}(D)
\end{align*}


==> sdp_lagrange.tex <==
Assume again that $\phi$ is the ReLU, and consider the box uncertainty set ${\cal U}^{\rm box}$~\cref{eq:U-def}. Our goal is to find the largest state discrepancy, measured in the Euclidean norm:
\[
p^* = \max_{x, \: u \in {\cal U}^{\rm box}} \: \|x-x^0\|_2^2 ~:~ x = z_+, \;\; z = Ax+Bu, \;\; |x-x^0| \le \sigma_x,
\]
We may use an SDP relaxation, based on a quadratic representation of $\phi$: for any two $n$-vectors $x,z$:
\begin{equation}\label{eq:phi-rep-quad}
x = \phi(z) \Longleftrightarrow x \ge 0, \;\; x \ge z, \;\; x \odot x \le x \odot z,
\end{equation}
where $\odot$ is the Hadamard (component-wise) product. 

% An equivalent, simpler condition involves just \emph{one} quadratic constraint:
% \begin{equation}\label{eq:phi-rep-quad-simple}
% x = \phi(z) \Longleftrightarrow x \ge 0, \;\; x \ge z, \;\; x^\top x \le x^\top z.
% \end{equation}

For a given $t \ge0$, the condition
$\|x-x^0\|_2^2 \le t$ holds whenever $x = \phi(Ax+Bu)$, $u \in {\cal U}$, $|x-x^0| \le \sigma_x$, if there exists $(\lambda,\mu,\nu,\eta,\kappa) \ge 0$ such that: for every $x,u$:
\begin{eqnarray*}
\|x-x^0\|_2^2 &\le& t + \sum_{i\in[n]} \lambda_i(x_i^2 - x_i(Ax+Bu)_i) - 2\mu^\top x - 2\nu^\top (x - (Ax+Bu)) \\
&& + \sum_{j=1}^p \eta_j ((u_j-u_j^0)^2 - \sigma_{u,j}^2) + \sum_{j=1}^n \kappa_j ((x_j-x_j^0)^2 - \sigma_{x,j}^2) \\
&=& t + x^\top (D_\lambda -\frac{1}{2}(D_\lambda A + A^\top D_\lambda))x -x^\top D_\lambda Bu \\&&
- 2\mu^\top x - 2\nu^\top (x - (Ax+Bu)) + (u-u^0)^\top D_\eta (u-u^0) - \sigma_u^\top D_\eta \sigma_u \\
&&+(x-x^0)^\top D_\kappa (x-x^0) - \sigma_x^\top D_\kappa \sigma_x,
\end{eqnarray*}
where, for a given vector $\alpha$, we denote $D_\alpha := \diag(\alpha)$.
The above can be written as $H(t, \lambda,\mu,\nu,\eta,\kappa) \succeq 0$, where
\begin{align*}
H(t, \lambda,\mu,\nu,\eta,\kappa) &: = 
\begin{pmatrix}
H_{xx} & H_{xu} & h_x \\
\ast & H_{uu} & h_u \\
\ast & \ast & h
\end{pmatrix} , \\
H_{xx} &:= D_\lambda -\frac{1}{2}(D_\lambda A + A^\top D_\lambda)- I , \;\;
H_{xu} := -\frac{1}{2}D_\lambda B , \;\; 
H_{uu} := D_\eta \\
h_x &:= -\mu-\nu+A^\top \nu+x^0-\frac{1}{2}D_\eta x^0  , \;\; h_u := -2D_\eta u^0+B^\top \nu \\
h &:= t - (x^0)^\top x^0 
+ (u^0)^\top D_\eta u^0 -\sigma_u^\top D_\eta \sigma_u 
+ (x^0)^\top D_\kappa x^0 -\sigma_x^\top D_\kappa \sigma_x.
\end{align*}
% and
% \begin{align*}
% \begin{pmatrix}
% D_\lambda -\frac{1}{2}(D_\lambda A + A^\top D_\lambda)- I & -\frac{1}{2}D_\lambda B&  \\
% \ast & D_\eta &  \\
% \ast & \ast & 
% \begin{array}{c}
% t - (x^0)^\top x^0 \\
% + (u^0)^\top D_\eta u^0 -\sigma_u^\top D_\eta \sigma_u \\
% + (x^0)^\top D_\kappa x^0 -\sigma_x^\top D_\kappa \sigma_x
% \end{array}
% \end{pmatrix} .
% \end{align*}
Observe that $H(\cdot)$ is a symmetric matrix that is affine in its arguments. The best upper bound that we can get this way is an SDP
\[
p^* \le \min_{t, \lambda,\mu,\nu,\eta,\kappa} \: t ~:~ H(t, \lambda,\mu,\nu,\eta,\kappa) \succeq 0, \;\; (\lambda,\mu,\nu,\eta,\kappa) \ge 0.
\]
% subsection sdp_relaxation (end)

% section robustness (end)

